SmartKC: Smartphone-based Corneal Topographer for Keratoconus Detection

Keratoconus is a severe eye disease affecting the cornea (the clear, dome-shaped outer surface of the eye), causing it to become thin and develop a conical bulge. The diagnosis of keratoconus requires sophisticated ophthalmic devices which are non-portable and very expensive. This makes early detection of keratoconus inaccessible to large populations in low- and middle-income countries, making it a leading cause for partial/complete blindness among such populations. We propose SmartKC, a low-cost, smartphone-based keratoconus diagnosis system comprising of a 3D-printed placido's disc attachment, an LED light strip, and an intelligent smartphone app to capture the reflection of the placido rings on the cornea. An image processing pipeline analyzes the corneal image and uses the smartphone's camera parameters, the placido rings' 3D location, the pixel location of the reflected placido rings and the setup's working distance to construct the corneal surface, via the Arc-Step method and Zernike polynomials based surface fitting. In a clinical study with 101 distinct eyes, we found that SmartKC achieves a sensitivity of 94.1% and a specificity of 100.0%. Moreover, the quantitative curvature estimates (sim-K) strongly correlate with a gold-standard medical device (Pearson correlation coefficient =0.78). Our results indicate that SmartKC has the potential to be used as a keratoconus screening tool under real-world medical settings.

==> tables/demographs.tex <==
\begin{table}[!tb]
\centering
 %\resizebox{\linewidth}{!}{
%\small
\begin{tabular}{ | c | c c c c |}
\toprule
\textbf{KT Case (N)} & \textbf{sim-K1} & \textbf{sim-K2} &  \textbf{PPK} & \textbf{Age}\\ 
\hline

No Keratoconus (33) & 45.20$\pm$1.78 D & 44.35$\pm$1.56 D & 0.02$\pm$0.02 & 24$\pm$4\\
Keratoconus (15) & 52.02$\pm$2.30 D & 48.15$\pm$1.71 D & 0.93$\pm$0.23 & 27$\pm$9\\

 \bottomrule
\end{tabular}
%}
\vspace{0mm}
\caption{Participant demographics.}

\label{tab:demographs}
\end{table}

==> tables/precision_recall_before_simkfix.tex <==
\begin{table}[!tb]
\centering
\caption{\imwutadd{Precision/Recall and Sensitivity/Specificity for \app{} and Keratron from the doctors' evaluation.\\
*: after removing retake, $^{\dagger{}}$: assuming if either eye (left/right) of a patient was marked as `keratoconus' both the eyes were evaluated as having `keratoconus'}}
\resizebox{\linewidth}{!}{
\small
\imwutadd{
\begin{tabular}{| c | c | c | c c c | c c |}
\toprule
\textbf{Examiner} & \textbf{System} & \textbf{\# of eyes}* & \textbf{Precision} & \textbf{Recall} & \textbf{F1 Score} & \textbf{Sensitivity} & \textbf{Specificity}\\ 
\hline
PPK  Metric & Keratron & 101 & 0.93 & 0.85 & 0.89 & 85.3\% & 97.0\%\\
\hline
Ophthalmologist \#1 & Keratron & 73 & 0.70 & 1.00 & 0.82 & 100.0\% & 66.1\% \\
Ophthalmologist \#1 & SmartKC & 86 & 0.96 & 0.87 & 0.91 & 87.1\% & 97.9\%\\
\hline
Ophthalmologist \#2 & Keratron & 61 & 0.93 & 1.00 & 0.96 & 100.0\% & 93.3\% \\
Ophthalmologist \#2 & SmartKC & 88 & 1.00 & 0.85 & 0.92 & 85.2\% & 100.0\%\\
%Ophthalmologist \#2 & SmartKC & 68 & 0.72 & 0.96 & 0.83 & 96.3\% & 73.2\%\\ This was before SimK correction
\hline
Combined & Keratron & 80 & 0.69 & 1.00 & 0.82 & 100.0\% & 68.1\% \\
Combined & SmartKC & 95 & 0.96 & 0.87 & 0.92 & 87.1\% & 98.4\%\\
%Combined & SmartKC & 90 & 0.74 & 0.88 & 0.81 & 87.8\% & 80.4\%\\ This was before SimK correction
\hline
Combined$^{\dagger{}}$ & Keratron & 80 & 0.69 & 1.00 & 0.82 & 100.0\% & 68.1\% \\
Combined$^{\dagger{}}$ & SmartKC & 95 & 0.94 & 0.94 & 0.94 & 93.5\% & 96.8\%\\
%Combined$^{\dagger{}}$ & SmartKC & 90 & 0.72 & 0.94 & 0.82 & 94.2\% & 76.5\%\\ This was before SimK correction 
 \bottomrule
\end{tabular}
}}
% \vspace{-4mm}

\label{tab:precision_recall}
%\vspace{-6mm}
\end{table}

% \app{} achieves a combined Sensitivity / Specificity of 85.7\% and 78.6\% as compared to gold standard device Keratron's Senstivity / Specificity of 100.0\% and 78.6\%, demonstrating \app{}'s efficacy in a clinical-setting.

==> tables/precision_recall_phase1.tex <==
\begin{table}[!h]
\centering
 \resizebox{\linewidth}{!}{
\small
\begin{tabular}{| c | c | c | c c c | c c |}
\toprule
\textbf{Examiner} & \textbf{System} & \textbf{\# of eyes}* & \textbf{Precision} & \textbf{Recall} & \textbf{F1 Score} & \textbf{Sensitivity} & \textbf{Specificity}\\ 
\hline
Ophthalmologist \#1 & Keratron & 40 & 0.70 & 1.00 & 0.82 & 100.0\% & 76.9\% \\
Ophthalmologist \#1 & SmartKC & 36 & 0.89 & 0.80 & 0.84 & 80.0\% & 96.2\%\\
\hline
Ophthalmologist \#2 & Keratron & 26 & 0.86 & 1.00 & 0.92 & 100.0\% & 85.7\% \\
Ophthalmologist \#2 & SmartKC & 36 & 0.60 & 0.90 & 0.72 & 90.0\% & 72.7\%\\
\hline
Combined & Keratron & 42 & 0.70 & 1.00 & 0.82 & 100.0\% & 78.6\% \\
Combined & SmartKC & 42 & 0.67 & 0.86 & 0.75 & 85.7\% & 78.6\%\\
 \bottomrule
\end{tabular}
}
% \vspace{-4mm}
\caption{Precision/Recall and Sensitivity/Specificity for \app{} and Keratron from the doctors' evaluation on the pilot study data.\\
% \app{} achieves a combined Sensitivity / Specificity of 85.7\% and 78.6\% as compared to gold standard device Keratron's Senstivity / Specificity of 100.0\% and 78.6\%, demonstrating \app{}'s efficacy in a clinical-setting.
*: after removing retake}

\label{tab:precision_recall_phase1}
\end{table}

==> tables/sim-error.tex <==
\begin{table}[!tb]
\centering
 %\resizebox{\linewidth}{!}{
%\small
\begin{tabular}{ |c | c c |}
\toprule
\textbf{Surface} & \textbf{Elevation Error} & \textbf{ROC Error}\\ 
\hline

Spherical & 0.07\% & 1.24\%\\
Ellipsoid & 0.04\% & 0.95\%\\
Zernike & 2.41\% & 3.25\%\\

 \bottomrule
\end{tabular}
%}
\vspace{0mm}
\caption{Mean percentage surface reconstruction error (in mm) for the reflection image from the simulated setup, for a spherical and an ellipsoidal artificial surface.}

\label{tab:sim-error}
\end{table}

==> tables/system-specs.tex <==
\begin{table}[!htbp]
\centering
 %\resizebox{\linewidth}{!}{
%\small
\begin{tabular}{ c c }
\toprule
\textbf{Parameter} & \textbf{Value}\\ 
\hline

Working Distance & 75.0 mm\\
Cone Length & 70.0 mm\\
Inner-Radius & 4.0 mm\\
Outer-Radius & 15.0 mm\\
Cone Semi-Verticle Angle & 8.93$^{\circ}$\\
Focal Length & 4.76 mm\\
Sensor Dimensions & 6.4 mm x 4.8 mm\\

 \bottomrule
\end{tabular}
%}
\vspace{0mm}
\caption{\textit{Optic specifications of the proposed system. Note: The Focal length and Sensor dimensions are given for the OnePlus 7T phone we have used for our experiments, but can be any other camera sensor.}}

\label{tab:system-specs}
\end{table}
